Convergence proofs and strong error bounds for forward-backward stochastic differential equations using neural network simulations

We introduce forward-backward stochastic differential equations, highlighting the connection between solutions of these and solutions of partial differential equations, related by the Feynman-Kac theorem. We review the technique of approximating solutions to high dimensional partial differential equations using neural networks, and similarly approximating solutions of stochastic differential equations using multilevel Monte Carlo. Connecting the multilevel Monte Carlo method with the neural network framework using the setup established by E et al. and Raissi, we provide novel numerical analyses to produce strong error bounds for the specific framework of Raissi. Our results bound the overall strong error in terms of the maximum of the discretisation error and the neural network's approximation error. Our analyses are necessary for applications of multilevel Monte Carlo, for which we propose suitable frameworks to exploit the variance structures of the multilevel estimators we elucidate. Also, focusing on the loss function advocated by Raissi, we expose the limitations of this, highlighting and quantifying its bias and variance. Lastly, we propose various avenues of further research which we anticipate should offer significant insight and speed improvements.

==> avenues_for_research.tex <==
\section{Avenues for research}

Having a multilevel Monte Carlo framework so naturally present itself in the context of neural networks, there are a few avenues of research that appear. At the crux of these are to try and use a small neural network as a coarse estimator, and a large neural network as a fine estimator. Additional to this, it is natural to suppose that for a regular multilevel Monte Carlo framework using differing temporal discretisations, that perhaps we can nest our neural network based multilevel Monte Carlo scheme within it, using the small neural network on the coarsest discretisation levels, and using the larger neural network on the finer discretisation. Conversely it might be more natural to nest the temporal discretisation within the neural network one. Whether one nesting should be better than the other is itself one interesting avenue for research. 

\subsection{Plan for research}

This is an MSc research project, and is consequently assessed using the following criteria, (which can be found at Imperial's ``\href{https://imperialcollege.atlassian.net/wiki/spaces/docteaching/pages/152420327/MSc+Individual+Projects}{MSc individual projects}'' webpage):
\begin{enumerate}[I.]
\item \label{item:literature_survey} Literature survey. 
\item \label{item:technical_work} Explain a technical or theoretical item and what was brought together to achieve this. For a pass grade, no original contribution is required, and for a distinction grade the work should cover some new ground. 
\item \label{item:evaluation} Evaluate the work performed. 
\end{enumerate}

With the basic premiss established, we have the following plan for our research:

\begin{enumerate}
\item Survey the literature for relevant research. 
\begin{itemize}
\item \Cref{sec:introduction} contains a moderately comprehensive collection of literature appropriate to our topic of research. So we believe we have a reasonable cross section of the literature to contrast and compare our work against, satisfying \cref{item:literature_survey}.
\end{itemize}

\item Replicate the results and setup of  \citet{raissi2018forwardbackward}.
\begin{itemize}
\item This will allow us to have a base numerical and computational setup to build off from, along with allowing us to verify the correctness of our setup. Furthermore, this will go some way to satisfying \cref{item:technical_work}. 
\end{itemize}

\item Replicate the results of \citet{guler2019robust}.
\begin{itemize}
\item This will allow us to review what they claimed as the MLMC setup, which I really suspect is just an iterative scheme and not an MLMC approach. 
\end{itemize}

\item Benchmark the computational costs seen. We know the training should be very expensive, as discussed by \citet{raissi2018forwardbackward}. However, we wish to verify that the neural network is the dominant cost to factor in when constructing any cost model, departing from the typical cost model (such as that by \citet{giles2008multilevel}) where the random number generation is the dominant cost. Should we verify our hypothesis, we can proceed onto the next stages of research. This will also safeguard us from red herrings coming from implementation details, such as e.g.\ verifying the dominant cost is evaluating the neural network, rather than copying the data on/off a GPU. 
\begin{itemize}
\item This is still relatively derivative (and a replication) of the work by \citet{raissi2018forwardbackward}, when considering \cref{item:technical_work}. However, experimental validation that the dominant cost is from neural network evaluation, rather than data movement across the CPU-GPU boundary, would be novel, albeit not very surprising. This would go some way towards demonstrating novel work for satisfying \cref{item:technical_work}.
\end{itemize}

\item Consider the computational costs that can be achieved by the nested multilevel Monte Carlo setting from a experimental point of view, and then if the results look encouraging, a theoretical analysis might be appropriate. 
\begin{enumerate}
\item Try to find a variance reduction in two and four way multilevel Monte Carlo difference terms. These are necessary if there is to be any recovery of potential cost savings. 
\item Computationally benchmark savings that can be realised. This will likely be in Python, but perhaps there might be C/C++ libraries available to make any savings more concrete or impressive. 
\item Compute the variance structure for a variety of payoffs/functionals which depend on the final process, which may include e.g.\ discontinuities, non-Lipschitz bounds, etc. 
\item Try to implement an end-to-end nested multilevel framework to show that it hopefully doesn't need to go to such high levels as that used by \citet{raissi2018forwardbackward}, and that computational savings can be had by adopting a nested multilevel approach. 
\item Should the numerics look semi-promising, then we may be able to utilise some of the numerical results from \citet{giles2022approximate} for analysing nested multilevel Monte Carlo schemes. If we can restrict ourselves to Lipschitz neural network activation functions and payoffs, then it might well be likely we can produce some analytic error bounds for the nested framework. 
\end{enumerate}
\begin{itemize}
\item If we are able to achieve any of these milestones, this would present a novel contribution, satisfying \cref{item:technical_work}
\end{itemize}

\item Review and evaluate our findings, and publish the work if appropriate. 
\begin{itemize}
\item When presenting our work, we would always do this and satisfy \cref{item:evaluation}. However, should the work look very promising, then the publication could be anything from an arXiv pre-print, to something perhaps suitable for SIAM, ACM, etc. 
\end{itemize} 
\end{enumerate}

\subsection{Other related areas of research}

While the bulk of the research proposed thus far appears to focus on the various bias and variance analysis for multilevel Monte Carlo applications, there are other directions we could pursue. 

\begin{itemize}
\item Try to formalise why one overall neural network is better than several disjunct ones for each time step. \citet{raissi2018forwardbackward} discusses this informally, but perhaps we can try tot formalise this somewhat. 

\item Try and learn corrections. Consider for example the Black-Scholes setup where we have learnt well everything for uncorrelated assets. Now consider a small perturbation of this and a system with small correlations between the assets. Can we learn how to correct for this. For the Black-Scholes setup we might have hope at some analytic results. This may be akin to using a control variate.

\item Focus on the bias and variance of the neural network, rather than the Euler-Maruyama scheme, and perhaps how these might couple. 
\end{itemize}

\subsection{Research items}

This is the TODO list of items that need investigating. 
\todo[inline=true, caption={}]{
\textbf{Offline isolated training}
\begin{itemize}
\item Replicate the results of \citet{raissi2018forwardbackward}.
\begin{itemize}
\item Check the errors are as we expect. 
\item Check the expensive bits are where we expect them to be. 
\item Check the expensive bits scale as we expect them to scale. 
\item Check we can easily enough save a learnt model. (to save time)
\end{itemize}

\item Replicate the results of \citet{guler2019robust}. 
\begin{itemize}
\item Check the exact framework is as we think it is (MLMC or otherwise?).
\item See if we can do it properly as a MLMC method (if not already). 
\end{itemize}
\end{itemize}

}

\todo[inline=true, caption={}]{
\textbf{Offline isolated training and inference}
\begin{itemize}
\item Building off the results from \citet{guler2019robust}, see if we can produce a nice MLMC framework.
\item Are the savings promising? 
\item Are there variance reductions promising?
\begin{itemize}
\item Are they all closely coupled?
\end{itemize}
\item Can we produce any analytic results?
\end{itemize}
}

\todo[inline=true, caption={}]{
\textbf{Online isolated training}
\begin{itemize}
\item Can we think of a good way to couple these and produce a MLMC that respects the telescoping sum?
\end{itemize}
}
